Vision Transformers for Small Histological Datasets Learned through Knowledge Distillation

Computational Pathology (CPATH) systems have the potential to automate diagnostic tasks. However, the artifacts on the digitized histological glass slides, known as Whole Slide Images (WSIs), may hamper the overall performance of CPATH systems. Deep Learning (DL) models such as Vision Transformers (ViTs) may detect and exclude artifacts before running the diagnostic algorithm. A simple way to develop robust and generalized ViTs is to train them on massive datasets. Unfortunately, acquiring large medical datasets is expensive and inconvenient, prompting the need for a generalized artifact detection method for WSIs. In this paper, we present a student-teacher recipe to improve the classification performance of ViT for the air bubbles detection task. ViT, trained under the student-teacher framework, boosts its performance by distilling existing knowledge from the high-capacity teacher model. Our best-performing ViT yields 0.961 and 0.911 F1-score and MCC, respectively, observing a 7% gain in MCC against stand-alone training. The proposed method presents a new perspective of leveraging knowledge distillation over transfer learning to encourage the use of customized transformers for efficient preprocessing pipelines in the CPATH systems.

==> extra/extra.tex <==

% Air bubbles are slide-level artifacts that occur when air is trapped under the cover slip due to improper mounting. They are primarily formed around the edge of a slide, but sometimes a bubble can appear in the middle in a tube-like shape. Bubbles might affect the scanning \cite{Shakhawat2020} and leave an altered and fainted appearance~\cite{Bindhu2013}.
% Shakhawat \etal~\cite{Hossain2018} experimented with detecting air bubbles for overall quality assessment of WSI. The task was carried out in two steps, where non-overlapping affected patches were first detected using an SVM classifier. Later, the remaining patches with fainted appearance were separated using four Gray-level co-occurrence matrix features. This work was extended in \cite{Shakhawat2020} to separate tissue artifacts from blur artifacts.
% Other than this, there is no literature available to the best of our knowledge that focuses on air bubbles. A possible reason could be that patches with fainted appearance are normalized with color processing methods described in the next section. 
% \par

% @incollection{pytorch,
% title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
% author = {Paszke, Adam and Gross, Sam and Massa, Francisco and Lerer, Adam and Bradbury, James and Chanan, Gregory and Killeen, Trevor and Lin, Zeming and Gimelshein, Natalia and Antiga, Luca and Desmaison, Alban and Kopf, Andreas and Yang, Edward and DeVito, Zachary and Raison, Martin and Tejani, Alykhan and Chilamkurthy, Sasank and Steiner, Benoit and Fang, Lu and Bai, Junjie and Chintala, Soumith},
% booktitle = {Advances in Neural Information Processing Systems 32},
% editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
% pages = {8024--8035},
% year = {2019},
% publisher = {Curran Associates, Inc.}}

==> extra/intro_old.tex <==
% Histopathology, the introduction of artifacts, air bubble, computational pathology, 
% DL for computational pathology
% CNN many parameters, overfits, and convolutions are expensive
% Vision transformers do well but require more data and do not generalize well on small datasets.
% Knowledge distillation helps in this gap.
% our contributions. 
\vspace{-0.5em}
Histopathological examination is the gold standard for assessing malignancy in the tissue sample under a microscope~\cite{khened2021generalized}. 
A pathologist's interpretation of diagnostic information relies on the quality of the histological glass slide. These glass slides are prepared using numerous laboratory procedures, which may introduce artifacts and variations causing loss of visual features~\cite{kanwal2022quantifying,taqi2018review}. Artifacts, such as air bubbles, occur when air is trapped under the cover slip due to improper mounting procedure~\cite{kanwal2022devil}. Eventually, the presence of air bubbles leaves an altered and fainted appearance~\cite{kanwal2022devil,taqi2018review}. Pathologists ignore regions containing artifacts as they are irrelevant for diagnosis. Therefore, it is important to consider this aspect while developing reliable Computer-aided Diagnostics (CAD).  \par 

Computational Pathology (CPATH) systems have the potential to automate diagnostic tasks and provide a second opinion by localizing the Regions of Interest (ROIs). However, the artifacts are ultimately transferred to the digitized version of the glass slide, called the Whole Slide Image (WSI)~\cite{kanwal2022devil}. CPATH systems, in the presence of histological artifacts, may result in wrong predictions. Deep Learning (DL) methods have shown promising results in various medical image analysis tasks~\cite{fuster2022invasive,tomasetti2022multi,wu2021quantifying}. Though, a preprocessing pipeline with DL models can ensure the automatic exclusion of air bubbles. Developing an efficient preprocessing pipeline is challenging as it requires  generalized DL models with high throughput. At the same time, developing generalized DL models requires a significant amount of data and labels, and the lack of sophisticated medical resources has always been a concern. Especially the patterns in histological images, which are infrequent such as artifacts. \par 

Deep Convolutional Neural Networks (DCNN) are popular for visual recognition tasks. DCNN detects complex representations by manipulating the texture features using convolutional filters. Though convolutions help learn inductive biases, they are expensive from a computational perspective. In addition, DCNN pays less significance to the global shape and focuses on texture features~\cite{geirhos2018imagenet}, which is troublesome in histopathology due to the stain variations. A recent trend of deploying ensembles of DCNN architectures with millions of parameters has been shown to improve the classification performance~\cite{beyer2020we}. Nonetheless, the use of complex ensembles is unviable for the preprocessing pipelines.  

After the success in natural language processing tasks, transformers have secured a bright spot in DL models for vision tasks~\cite{dosovitskiy2020image,kanwal2022attention}. Thanks to multi-head attention~\cite{vaswani2017attention}, which helps Vision Transformers (ViTs) to interact with the global shape and rely less on texture features. Unlike the convolution layer in DCNNs, which applies the same filter weights to all inputs, the multi-attention in ViTs attends to image-wide structural information~\cite{naseer2021intriguing}. Interestingly, ViTs are shown to be much more robust and generalized than DCNNs~\cite{bhojanapalli2021understanding,naseer2021intriguing}; Unfortunately, the robustness and generalizability come from training on extremely large datasets~\cite{bhojanapalli2021understanding,dosovitskiy2020image}, which leads us to the question like, are we done with the vision transformer for medical image analysis?

% contrasts with most biomedical scenarios. It
% for out-of-distribution samples, and CNN are content-independent, transformers have content-dependant long-range interation[naseer2021intriguing] 
% ~\cite{bai2021transformers}. 
% CNN has shape bias [ritter et al.]
% Transfer learning helps to cover insufficient data, but ImageNet pretrained DCNN carries a strong texture bias[Geirhos et al. 2019]. 

Transfer learning has been widely used to cope with the limitation of insufficient medical data. Unfortunately, pretrained weights are unavailable for customized architectures, and ImageNet~\cite{imagenet} weights carry a strong texture bias~\cite{geirhos2018imagenet}. In the urge to overcome these limitations, Knowledge Distillation (KD)~\cite{hinton2015distilling} methods have recently received attention from the biomedical imaging community. KD fills the gap by transferring learned knowledge from a large DL model to a lightweight one, making it suitable for preprocessing pipeline in the CPATH system. In other words, the knowledge can be distilled from a cumbersome DCNN teacher with better learning abilities to a student ViT model, overcoming the generalization problem caused by smaller medical datasets. 

Motivated by the KD results, we present a student-teacher recipe, as shown in Fig~\ref{fig:intro}, for training a transformer-based student architecture using a DCNN teacher. Our objective is to train a small vision transformer for air bubbles detection that performs better than the same model-trained standalone. To the best of our knowledge, the student-teacher framework using a ViT for air bubbles detection has not yet been proposed. Our contributions in this paper can be summarized as follows:

% \vspace{-2em}
\begin{figure}[ht!]
    \centering
    \includegraphics[width=1.1\textwidth]{images/main_v3.pdf}
    \vspace{-1.5em}
    \caption{\textbf{An introductory overview of our air bubbles detection method:} Predefined size patches for air bubbles, and artifact-free classes are extracted from the Whole Slide Image (WSI). A Vision Transformer (ViT) student model is trained with the help of a Deep Convolutional Neural Network (DCNN) teacher model by leveraging the transference of knowledge during the training process. The student-teacher recipe weights the teacher and student's outputs by the temperature (T) and adds knowledge beyond labels. The overall training objective is to minimize the final loss, which is a linear combination of student loss and distillation loss. Finally, the student model is used to perform prediction for binary air bubbles detection task. \vspace{-1.25em}}
    \label{fig:intro}
\end{figure}

\begin{itemize}[wide]
\item We train several DCNNs and ViTs to compare their performance on a binary air bubbles detection task. Later, we choose suitable to test our student-teacher framework. 
\item We conduct a fair and in-depth comparison by initializing ViT with and without pretrained weights and training it under a standalone vs. student-teacher framework.
\item We run extensive experiments to test the ViT's performance under different teacher models and distillation configurations on unseen data.   
\end{itemize}



==> extra/method_old.tex <==
% Preliminaries 
\vspace{-0.5em}
Fig.~\ref{fig:intro} provides an overview of our air bubbles detection method using KD~\cite{hinton2015distilling} in a student-teacher recipe where we propose to use a complex DCNN as the pre-trained teacher and a small ViT as the student when only a small histological dataset is available. We are doing a logit-based distillation~\cite{meng2021knowledge} since our teacher and student models are very different. 

%Fig.~\ref{fig:intro} provides an overview of our air bubbles detection method using the student-teacher recipe. We are re-purposing the KD method~\cite{hinton2015distilling} to generalize the classification performance of ViTs on a small histological dataset. Our approach aims to train a ViT under the guidance of a teacher (DCNN) model, where the student (ViT) model optimizes its learning by absorbing the additional knowledge from the teacher beyond labels.  The steps of this recipe are described below. 



%\paragraph{\textbf{Step 1:}} 
\subsection{Foreground Segmentation and Patching}
Let $I_{\text{WSI}(i)}^{40x}$ correspond to a WSI at magnification level 40x (sometimes referred to as 400x).  $I_{\text{WSI}}^{40x}$ are very large gigapixel images, and it is not feasible to process the entire WSI at once. As such, all  CPATH systems resort to patching or tiling of the image, or the ROI in the image, before further processing. Let ${\cal T} : I_{\text{WSI(i)}\in R}^{40x} \rightarrow \{{\bf x}_{j}^{i}; j=1\cdots J \}$ represent the process of patching a region defined by $R$ of the image $I_{\text{WSI}(i)}^{40x}$ into a set of $J$ patches, where  $\bx_j^{i}\in\mathbb{R}^{W\times H \times C}$ and $W$, $H$, $C$ present the width, height, and channels of the image, respectively. In the patching process, foreground-background segmentation was first performed by transforming RGB images to HSV color space Otsu thresholding was applied to the values channel to obtain the foreground containing tissue. The extracted foreground was later divided over a non-overlapping square grid, and patches with 70\% overlap to the annotation region ($R$) were extracted.   

Let $\mathcal{D}=(\bX, \by) = \{(\bx_n,\by_n)\}_{n=1}^{N}$ denote our prepared dataset of N patches from a set of WSI´s and $y_n\in\{0,1\}$ is the binary ground truth for the $n$-th instance, where 1 indicates a patch within a region marked as air bubbles. Fig~\ref{fig:intro} (step 1) shows the patches ($\bx_{n}$) of $224\times224\times3$ pixels, obtained from a WSI at 40x magnification.

% WSIs are too big to process in memory all at once; therefore, the patches of $224\times224$ pixels are extracted from WSI at 40x magnification. During the patching process, the foreground-background segmentation was conducted in the first stage using a combination of Otsu and binary thresholding on the HSV-transformed image. The extracted foreground was later divided on a square grid, and patches with a 70\% overlap to the annotation mask were extracted.
% The extracted foreground was later used to create patches with a 70\% overlap to the annotation mask.

%  Tissue masks were generated using HSV format to locate the blue and magenta color range, cor-
% responding to H&E stained tissue areas. The color range, hue, of WSIs in the HSV format was set to 100-180. Closing and opening
% morphological operations were applied to lesion masks to remove small regions and fill small holes, respectively, giving
% the final tissue-region R used in further processing.

\subsection{Selecting Student-Teacher Architectures}
Let`s symbolize the student model ($\S$) with parameters ($\theta$), providing the prediction output logits $\s_{n}=\S_{\theta}(\bx_{n})$, and correspondingly,  the teacher model ($\T$) parameterized by $\phi$ providing the output logits $\t_{n}=\T_{\phi}(\bx_{n})$.

Our student model is a ViT, similar to the pioneering work~\cite{dosovitskiy2020image}, which leverages multi-head self-attention mechanism~\cite{vaswani2017attention} to capture content-dependant relations across the input patch. At the image pre-processing layer, the patches of $224\times224$ pixels are split into the non-overlapping cells of $16\times16$ pixels. Later, the linear embedding layer flattens these cells, and positional encodings are added before feeding the embeddings to the pile of transformer blocks, as illustrated in Fig.~\ref{fig:intro}(see 2). Since convolutional networks have shown their efficacy in image recognition tasks, the Transfer of knowledge from a DCNN network can help the ViT absorb high shape and texture bias simultaneously~\cite{naseer2021intriguing}. Therefore, we rely on popular state-of-the-art DCNNs for selecting teacher architecture. Nevertheless, We systemically discover appropriate student and teacher candidate architectures during the experiments later to demonstrate the approach's effectiveness over the transfer learning.

% we rely on a set of the four popular state-of-the-art DCNNs for selecting teacher architecture.

% The teacher model $\T$ parameterized by $\phi$ will provide the output logits $\t_{n}=\T_{\phi}(\bx_{n})$, and correspondingly the student model $\S$ is parameterized by $\theta$ providing the prediction output logits $\s_{n}=\S_{\theta}(\bx_{n})$. 

\subsection{Training Student under Knowledge Distillation}
After selecting student and teacher architectures, we begin the process of training the student model. The goal is to train $\S$ with the assistance of a cumbersome $\T$ to improve the $\S$`s generalization performance using additional knowledge beyond the labels. Our approach is similar to Hinton \etal~\cite{hinton2015distilling} where model outputs $\s$, and $\t$ are normalized by a temperature ($\temp$) parameter before using the softmax function ($\sigma$). In short, the increasing value of $\temp$ softens the impact of the fluctuations in the output probability distribution, and more knowledge can be devolved with each input $\bx_{n}$. 
Instead of using softmax on $\s_{n}$, we take advantage of the log-softmax function ($\sigma^*$), which stabilizes the distillation process by heavily penalizing for incorrect class. $\sigma^*$ also adds efficiency to the training process by optimizing gradient calculations. 


%For an input patch ($\bx$), the output class probabilities from $\S$ and $\T$ can be defined as~\eqref{eq:1} and~\eqref{eq:2}, where $c$ is the total number of classes and $c_{i}$ denotes class i.

%\begin{equation}
%p_{\S{i}}=p(c_{i}|\bx ; \theta,T)
%\end{equation}
%\begin{equation} 
%p_{\T}=p(\hat{\by}_{t}|\bx ; \phi,T)
%\end{equation}

The output logits for input patch $\bx_{n}$ can be written as; 

\begin{equation}\label{eq:1}
\s_{n}=\S_{\theta}(\bx_{n}) \quad \textrm{and} \quad \t_{n}=\T_{\phi}(\bx_{n})
\end{equation}

Let the softmax and log-softmax on logits, $\sigma^*(\s/\temp)$ and $\sigma(\t/\temp)$, for each element can be defined as; 
\begin{equation} \label{eq:2}
    \sigma^*(s_{i}/\temp) = \frac{\exp{(s_{i}/\temp)}}{\sum_{j=1}^{c}\exp{(s_{j}/\temp)}}
\end{equation}
where T is the temperature often put to 1. 
The class probabilities at the output of the student model can thus be written as:
\begin{equation} \label{eq:1}
    p_{\S}=\sigma(\s/\temp) = \sigma(\S_{\theta}(\bx))
\end{equation}

% \begin{equation} \label{eq:1}
%     p_{\S_{i}}=\sigma(s_{i}/\temp) = \frac{\exp{(s_{i}/\temp)}}{\sum_{j=1}^{c}\exp{(s_{j}/\temp)}}
% \end{equation}
% \vspace{-0.5em}
% \begin{equation} \label{eq:2}
%  p_{\T_{i}}=\sigma^*(t_{i}/\temp) =\log\biggl(\frac{\exp{(t_{i}/\temp)}}{\sum_{j=1}^{c}\exp{(t_{j}/\temp)}}\biggl)
% \end{equation}


% \begin{equation} \label{eq:1}
%     p_{\S} = p(\bx_i|\Theta) = \frac{\exp{(\s_{i}/\temp)}}{\sum_{j}\exp{(\s_{i}/\temp)}} \quad \texttrm{and} \quad  p_{\T} = p(\bx_i|\phi) = \log\frac{\exp{(\t_{i}/\temp)}}{\sum_{j}\exp{(\t_{i}/\temp)}}
% \end{equation}
% \vspace{-0.5em}
% \begin{equation} \label{eq:1}
%     p_{\S} = p(\bx_i|\Theta) = \sigma(\s_{i}/\temp) = \frac{\exp{(\s_{i}/\temp)}}{\sum_{j}^{c}\exp{(\s_{j}/\temp)}}
% \end{equation}
% \vspace{-0.5em}
% \begin{equation} \label{eq:2}
%     p_{\T} = p(\bx_i|\phi) = \sigma^*(\t_{i}/\temp) =\log\biggl(\frac{\exp{(\t_{i}/\temp)}}{\sum_{j}^{c}\exp{(\t_{j}/\temp)}}\biggl)
% \end{equation}


 The student loss (eq.~\eqref{eq:student}) provides hard targets and is obtained by applying cross entropy ($L_{CE}$) on ground truth ($y$), and  $\sigma$ to $\s$:
 \begin{equation} \label{eq:student}
    L_{student} = L_{CE}(y, \sigma(\s)) = -\sum_{i=1}^{c} y_{i} \cdot log(p_{{\S}_{i}})
\end{equation}
Distillation loss provides the soft targets and is computed from the $p_{\S}$ and $p_{\T}$ by applying Kullback-Leibler divergence ($KL_{D}$). Since the outputs from $\S$ and $\T$ were normalized by $\temp$, we multiply the loss with $\temp^2$ to maintain their relative contribution :
\begin{equation} \label{eq:distillation}
    L_{distillation} = {T}^2 \times KL_{D} (p_{\S} \| p_{\T})= {T}^2 \cdot \sum_{i=1}^{c} p_{{\S}_{i}} log\frac{p_{{\S}_{i}}}{p_{{\T}_{i}}}
\end{equation}
 The final loss function, as shown in eq.~\eqref{eq:floss}, is a weighted average of student and distillation losses. 
\begin{equation} \label{eq:floss}
    L_{Final} = \alpha \times L_{student}  +  \beta \times L_{distillation}    \quad  \cdot :  \beta = 1-\alpha
\end{equation}
\vspace{-1em}
% \begin{equation} \label{eq:student}
%     L_{student} = L_{CE}(y, \sigma(\s)) = -\sum_{i=1}^{c} y_{i} \cdot log(p_{{\S}_{i}})
% \end{equation}
% \vspace{-1em}
% \begin{equation} \label{eq:distillation}
%     L_{distillation} = {T}^2 \times KL_{D} (p_{\S} \| p_{\T})= {T}^2 \cdot \sum_{i=1}^{c} p_{{\S}_{i}} log\frac{p_{{\S}_{i}}}{p_{{\T}_{i}}}
% \end{equation}


 High entropy in soft targets offers significantly more information per training patch than hard targets~\cite{hinton2015distilling}, allowing ViT to train with fewer data and a higher learning rate. Therefore, using a smaller alpha can be beneficial if the $\S$ is trained from scratch. 

%\paragraph{\textbf{Step 4:}} 
\subsection{Inference/prediction}
Once the final loss is minimized based on the experimental setup (defined in sec.~\ref{sec:experiment}), we find predictions from the student model $\S$ by putting $\temp$ equal to one. For a test patch ($\textbf{x}_*$), output can be defined as~\eqref{eq:pred}
\vspace{-0.5em}
%\begin{equation} \label{eq:pred}
    %p_{\S}(\textbf{x}= p(\textbf{x}_*|\Theta)
%     \hat{y}_{s} = \argmax\biggl( \frac{\exp{(\s_{i})}}{\sum_{j}^{c}\exp{(\s_{j})}}\biggl) \quad   \in \ \{0,1\}
% \end{equation}
\begin{equation}
       \hat{y}_{s} = \argmax(\sigma(\s))=\argmax(\sigma(\S_{\theta}(\bx))) \quad   \in \ \{0,1\}
\end{equation}


% Hinton suggests putting low weights on student loss gives best results, we find the same

% originally proposed KD to train small models with the help of high-capacity ensembles of large models.  
% by leveraging the transference of knowledge from a teacher network to a student network
% train a student (ViT) model, leveraging the training process using the  knowledge acquired by the teacher.

% Knowledge distillation (KD) helps to replace an ensemble of models by training a new one in a teacher-student paradigm. The student model is a small network trained from scratch, and the teacher model is an extensive large network helping students learn better. KD also aims to perform model compression to find a small model which is deployable and equally generalizable. 

% Knowledge is transferred from the teacher network to the student network by minimizing the loss function and applying softmax temperature (T). The probability pi of class ii is calculated from the teacher logits z as:
% pi=exp(zi/T)/∑jexp(zj/T)
% Softmax calculated to find a high value for maximum logit and pushed other probabilities toward zero. 

%To make this distribution softer, the temperature is introduced. With a softened distribution, each training input provides more knowledge and gradient for different inputs and does not fluctuate. So the student model can be trained with fewer data and a higher learning rate.  In other words, the increasing value of T softens the impact of the output probability distribution from the teacher model, the temperature determines how much-hidden knowledge needs to be transferred from the teacher to the student—higher temperature results in giving more importance to soft labels. Therefore, a lower temperature works better as the student model is smaller than the teacher model. 


% Distillation loss is calculated from the teacher`s probabilities and the student`s probabilities using a loss function.  
% Student loss is calculated with standard softmax function from hard predictions and ground truth.
% Final Loss = alpha * student loss + beta *distillation loss 		 :. Beta = 1- alpha	
% Using minor alpha compared to the beta can be beneficial as the student network starts from scratch.

% When the soft targets have high entropy, they provide much more information per training case than hard targets and much less variance in the gradient between training cases.


 % log softmax: By using the log-softmax, the model training efficiency can be greatly increased while reducing the training time. This is because we need to do fewer arithmetic operations while computing the gradients. Because log-softmax is a log over probabilities, the probabilities do not get very small. These advantages can be extremely important for implementation, especially when training a model can be computationally challenging and expensive. At the heart of using log-softmax over softmax is using log probabilities over probabilities, which has nice information theoretic interpretations.

==> extra/table2_old.tex <==
\begin{table}[ht!]
\centering
\renewcommand{\arraystretch}{1.5}
\caption{\textbf{Results From Experiment 2}: Knowledge Distillation (KD) outcome for selected teacher and student candidates from the previous experiment. Two teachers (VGG16 and MobileNet) with pretrained knowledge of air bubbles are used. While MobileNet is also initialized with knowledge of other domains to evaluate the teacher's influence. The best metrics are marked in bold.}

 \begin{tabular}{l| c c c| c c c}
 \hline
 \multicolumn{1}{|c}{}  & \multicolumn{3}{|c|}{\textbf{Validation Set}} & \multicolumn{3}{c|}{\textbf{Test Set}} \\
\cline{2-7}

\multicolumn{1}{|c}{\multirow{-2}{*}{Baseline (Initial.)}} & \multicolumn{1}{|c}{Acc.(\%)} & \multicolumn{1}{|c}{F1} & \multicolumn{1}{|c}{MCC($\Uparrow$)} & \multicolumn{1}{|c}{Acc.(\%)} & \multicolumn{1}{|c}{F1} & \multicolumn{1}{|c|}{MCC($\Uparrow$)}\\


  \Xhline{3\arrayrulewidth}
     {ViT-tiny (Scratch) & 96.13 & 0.963 & 0.922 & 91.51 & 0.925& 0.829   \\
     {ViT-tiny (ImageNet~\cite{imagenet}) & 98.67 & 0.987 & 0.973 & 92.35 & 0.933 & 0.847\\[0.2em]
   \Xhline{2\arrayrulewidth}
 \end{tabular}
 
\begin{tabular}{l| c c c |c c c}
    \hline
    % \cline{3-8}

    \multicolumn{1}{|c|}{{Teacher (Initial.)}} & Acc.(\%) & \multicolumn{1}{|c}{F1} & \multicolumn{1}{|c}{MCC($\Uparrow$)} & \multicolumn{1}{|c}{Acc.(\%)} & \multicolumn{1}{|c}{F1} & \multicolumn{1}{|c|}{MCC($\Uparrow$)} \\
    % \multicolumn{1}{|c}{\multirow{-2}{*}{Teacher}} & \multicolumn{1}{|c}{\multirow{-2}{*}{Initial.}} & \multicolumn{1}{|c}{\multirow{-2}{*}{$\alpha, T$}} & \multicolumn{1}{|c|}{Acc.(\%)} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{MCC($\Uparrow$)} & \multicolumn{1}{c|}{Acc.(\%)} & \multicolumn{1}{c|}{F1} & \multicolumn{1}{c|}{MCC($\Uparrow$)} \\
    
    \Xhline{3\arrayrulewidth}
    MobileNet (Scratch) & 98.73 & 0.988 & 0.974 & 93.38 & 0.941 & 0.866 \\
    MobileNet (ImageNet~\cite{imagenet}) & 98.56 & 0.987 & 0.972 & 93.38 & 0.942 & 0.867\\
    MobileNet (Damaged~\cite{kanwal2022quantifying}) & 50.08 & 0.211 & 0.09 & 35.51 & 0.116 & -0.294 \\
    MobileNet (Air bubbles) & 98.61 & 0.986 & 0.972 & 95.60 & 0.961 & 0.911 \\
    VGG16 (Air bubbles) & 98.67 & 0.987 & 0.973 & 94.19 & 0.948 & 0.882 \\[0.2em]
    \Xhline{2\arrayrulewidth}
 \end{tabular}
 
% \begin{tablenotes}
%     \item[1] Baseline Models without ImageNet initialization
%     \item[2] Baseline Models with ImageNet initialization
% \end{tablenotes}
    \label{res:2}
\end{table}
